On the information-theoretic structure of distributed measurements

The internal structure of a measuring device, which depends on what its components are and how they are organized, determines how it categorizes its inputs. This paper presents a geometric approach to studying the internal structure of measurements performed by distributed systems such as probabilistic cellular automata. It constructs the quale, a family of sections of a suitably defined presheaf, whose elements correspond to the measurements performed by all subsystems of a distributed system. Using the quale we quantify (i) the information generated by a measurement; (ii) the extent to which a measurement is context-dependent; and (iii) whether a measurement is decomposable into independent submeasurements, which turns out to be equivalent to context-dependence. Finally, we show that only indecomposable measurements are more informative than the sum of their submeasurements.

==> eptcsdata.tex <==
\providecommand{\firstpage}{28}
\providecommand{\publicationstatus}{E. Kashefi, J. Krivine, F. van Raamsdonk (Eds.) \\
DCM 2011\\
EPTCS 88, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.88.3}{10.4204/EPTCS.88.3}}
\pdfoutput=1

